Topology-Matching Normalizing Flows for Out-of-Distribution Detection in Robot Learning

To facilitate reliable deployments of autonomous robots in the real world, Out-of-Distribution (OOD) detection capabilities are often required. A powerful approach for OOD detection is based on density estimation with Normalizing Flows (NFs). However, we find that prior work with NFs attempts to match the complex target distribution topologically with naive base distributions leading to adverse implications. In this work, we circumvent this topological mismatch using an expressive class-conditional base distribution trained with an information-theoretic objective to match the required topology. The proposed method enjoys the merits of wide compatibility with existing learned models without any performance degradation and minimum computation overhead while enhancing OOD detection capabilities. We demonstrate superior results in density estimation and 2D object detection benchmarks in comparison with extensive baselines. Moreover, we showcase the applicability of the method with a real-robot deployment.

==> main/4_1_table_results.tex <==
% softmax
\def\VocSAuroc{$0.901$}
\def\VocSFprA{$72.8$}
\def\VocSFprB{$83.1$}
\def\CoSAuroc{$0.882$}
\def\CoSFprA{$70.6$}
\def\CoSFprB{$78.1$}
\def\YSAuroc{$0.884$}
\def\YSFprA{$47.7$}
\def\YSFprB{$91.2$}
% entropy
\def\VocEAuroc{$0.905$}
\def\VocEFprA{$72.9$}
\def\VocEFprB{$82.9$}
\def\CoEAuroc{$0.903$}
\def\CoEFprA{$70.6$}
\def\CoEFprB{$80.2$}
\def\YEAuroc{$0.885$}
\def\YEFprA{$47.6$}
\def\YEFprB{$91.2$}
% ensemble softmax
\def\VocESAuroc{$0.885$}
\def\VocESFprA{$72.6$}
\def\VocESFprB{$83.1$}
\def\CoESAuroc{$0.898$}
\def\CoESFprA{$73.5$}
\def\CoESFprB{$82.3$}
\def\YESAuroc{$0.898$}
\def\YESFprA{$73.5$}
\def\YESFprB{$82.3$}
% ensemble entropy
\def\VocEEAuroc{$0.887$}
\def\VocEEFprA{$72.5$}
\def\VocEEFprB{$83.1$}
\def\CoEEAuroc{$0.906$}
\def\CoEEFprA{$73.5$}
\def\CoEEFprB{$82.3$}
\def\YEEAuroc{$0.906$}
\def\YEEFprA{$73.5$}
\def\YEEFprB{$82.3$}
% gmmdet
\def\VocGDAuroc{$0.931$}
\def\VocGDFprA{$80.5$}
\def\VocGDFprB{$89.3$}
\def\CoGDAuroc{$0.924$}
\def\CoGDFprA{$80.2$}
\def\CoGDFprB{$87.9$}
\def\YGDAuroc{$0.894$}
\def\YGDFprA{$56.7$}
\def\YGDFprB{$87.4$}
% ensemble gmmdet
\def\VocEGDAuroc{$0.920$}
\def\VocEGDFprA{$79.6$}
\def\VocEGDFprB{$85.7$}
\def\CoEGDAuroc{$0.927$}
\def\CoEGDFprA{$\textbf{84.7}$}
\def\CoEGDFprB{$89.5$}
\def\YEGDAuroc{$0.927$}
\def\YEGDFprA{$\textbf{84.7}$}
\def\YEGDFprB{$89.5$}
% flow gaussian
\def\VocFGAuroc{$0.915\pm0.23$}
\def\VocFGFprA{$77.5\pm0.23$}
\def\VocFGFprB{$85.7\pm0.23$}
\def\CoFGAuroc{$0.925\pm0.23$}
\def\CoFGFprA{$82.4\pm0.23$}
\def\CoFGFprB{$89.5\pm0.23$}
\def\YFGAuroc{$0.925\pm0.23$}
\def\YFGFprA{$82.4\pm0.23$}
\def\YFGFprB{$89.5\pm0.23$}
% flow gmm
\def\VocFGMAuroc{$0.918\pm0.23$}
\def\VocFGMFprA{$73.9\pm0.23$}
\def\VocFGMFprB{$84.8\pm0.23$}
\def\CoFGMAuroc{$0.925\pm0.23$}
\def\CoFGMFprA{$81.9\pm0.23$}
\def\CoFGMFprB{$89.5\pm0.23$}
\def\YFGMAuroc{$0.925\pm0.23$}
\def\YFGMFprA{$81.9\pm0.23$}
\def\YFGMFprB{$89.5\pm0.23$}
% flow rsb
\def\VocFRAuroc{$0.921\pm0.23$}
\def\VocFRFprA{$78.1\pm0.23$}
\def\VocFRFprB{$85.9\pm0.23$}
\def\CoFRAuroc{$0.924\pm0.23$}
\def\CoFRFprA{$81.8\pm0.23$}
\def\CoFRFprB{$89.3\pm0.23$}
\def\YFRAuroc{$0.924\pm0.23$}
\def\YFRFprA{$81.8\pm0.23$}
\def\YFRFprB{$89.3\pm0.23$}
% flow gmm cls
\def\VocFGMCAuroc{$0.922\pm0.23$}
\def\VocFGMCFprA{$77.2\pm0.23$}
\def\VocFGMCFprB{$86.4\pm0.23$}
\def\CoFGMCAuroc{$0.924\pm0.23$}
\def\CoFGMCFprA{$81.8\pm0.23$}
\def\CoFGMCFprB{$89.3\pm0.23$}
\def\YFGMCAuroc{$0.924\pm0.23$}
\def\YFGMCFprA{$81.8\pm0.23$}
\def\YFGMCFprB{$89.3\pm0.23$}
% flow rsb cls
\def\VocFRCAuroc{$0.918\pm0.23$}
\def\VocFRCFprA{$78.9\pm0.23$}
\def\VocFRCFprB{$87.2\pm0.23$}
\def\CoFRCAuroc{$0.926\pm0.23$}
\def\CoFRCFprA{$81.5\pm0.23$}
\def\CoFRCFprB{$89.1\pm0.23$}
\def\YFRCAuroc{$0.926\pm0.23$}
\def\YFRCFprA{$81.5\pm0.23$}
\def\YFRCFprB{$89.1\pm0.23$}
% flow gmm ib
\def\VocFGIAuroc{$0.934\pm0.23$}
\def\VocFGIFprA{$79.9\pm0.23$}
\def\VocFGIFprB{$87.9\pm0.23$}
\def\CoFGIAuroc{$0.924\pm0.23$}
\def\CoFGIFprA{$79.1\pm0.23$}
\def\CoFGIFprB{$89.2\pm0.23$}
\def\YFGIAuroc{$0.924\pm0.23$}
\def\YFGIFprA{$79.1\pm0.23$}
\def\YFGIFprB{$89.2\pm0.23$}
% flow rsb ib
\def\VocFRIAuroc{$\textbf{0.945}\pm0.23$}
\def\VocFRIFprA{$\textbf{84.3}\pm0.23$}
\def\VocFRIFprB{$\textbf{90.6}\pm0.23$}
\def\CoFRIAuroc{$\textbf{0.934}\pm0.23$}
\def\CoFRIFprA{$\textit{84.1}\pm0.23$}
\def\CoFRIFprB{$\textbf{91.6}\pm0.23$}
\def\YFRIAuroc{$\textbf{0.934}\pm0.23$}
\def\YFRIFprA{$\textit{84.1}\pm0.23$}
\def\YFRIFprB{$\textbf{91.6}\pm0.23$}

==> main/method_old.tex <==
\section{Method}
\label{methods}

%Our method for \gls{ood} detection in the demanding realm of Open-Set Object Detection is well-suited for mobile applications due to its resource efficiency. 
Before we introduce our main method and describe how it overcomes the topological mismatch, in \Cref{tp_problem}, we will first formalize the setting. Last, in \Cref{inference}, we describe specifics about how the resulting Normalizing Flow is used for \gls{ood} detection.
%\gls{ood} detection in the realm of Open-Set Object Detection is key for many real-world robotic perception~\cite{feng2022bayesian, lee2022virtual}. Our method   Therefore, we start with the problem formulation in this context and then introduce the problem of topological mismatch in \gls{nf} and the proposed method to address it. 


% We argue that gls{ood} detection for Object Detection is more challenging than, e.g., the traditionally studied task of image classification. Specifically, in Object Detection, we deal with structured predictions with multiple objects in a single image. As we are going to show, for methods using \gls{nf}, there is the important problem of topological mismatch left unattended in prior work. This comes with adverse theoretical and practical implications. Before going into more detail about the topological mismatch introducing our main method, in \Cref{tp_problem}, for detecting \gls{ood} in the context of Open-Set Object Detection~\cite{miller2021uncertainty, Dhamija_2020_WACV} we will first formalize the setting. Last, in \Cref{inference}, we describe specifics about how the resulting Normalizing Flow is used for \gls{ood} detection.

%We start with the problem formulation of \gls{ood} detection in the context of Open-Set Object Detection~\cite{miller2021uncertainty, Dhamija_2020_WACV}, which is more relevant to real-world robotic perception~\cite{lee2022virtual, feng2022bayesian}.
%The goal is to train an object detector that can not only localize and categorize the known objects seen during training but also \textit{identify unknown objects} unseen during training but falsely detected during test-time.
% This is more challenging than image classification due to the fine-grained reasoning on object-level instead of image-level and the necessary requirement of real-time inference, which is meanwhile beneficial for robots in need of timely decision-making. 
%We aim to achieve such object detector with a topologically matched \gls{nf} trained with \gls{ib} due to several appealing properties of \gls{nf} such as its easy compatibility with existing models and the fast inference with only single forward pass.
%In the following, we will first introduce the problem, briefly describe the fundamental topological constraint of \gls{nf} and elaborate how we employ expressive base distributions to mitigate this problem.

\paragraph{Problem Formulation} 
\def\flowNum{n}
\def\baseParam{\psi}
\def\baseVarCap{Z}
\def\baseVar{\bb{z}}
\def\flowFunc{T}
\def\subflowFunc{t}
\def\flowParam{\phi}
\def\oodFunc{h}
\def\featDim{d} 
\def\featVarCap{U}
\def\featVar{\bb{u}}
\def\detFunc{F} 
\def\detParam{\theta} 
\def\backboneFunc{f} 
\def\clsFunc{g}
% We define a data-set $\mathcal{D}_{id}=\{ (\bb{x}_i, \bb{b}_i, y_i) \}_{i=1}^{N}$ consisting of $N$ samples of objects with corresponding object bounding box coordinates $\bb{b}_i \in \mb{R}^4$ and class label $y_i \in \mb{Y} = \{1,2,...,C\}$ on an image $\bb{x}_i \in \mb{X}_{id}$ drawn from some known distribution $\mb{P}_{id}=\mb{X}_{id} \times \mb{Y} \times \mb{R}^4$. 
Given an image $\bb{x}_i \in \mb{X}$, a trained object detector $\detFunc_\detParam = \backboneFunc_\detParam \circ \clsFunc_\detParam$ parameterized by $\detParam$ would localize and classify the objects of interests specified by bounding box coordinates $\bb{b}_i \in \mb{R}^4$ and class label $y_i \in \mb{Y} = \{1,2,...,C\}$ drawn from some known distribution $\mb{P}_{id}$. 
% where there is one module for both bounding box prediction and feature extraction $\backboneFunc_{\detParam}: \mb{X}_{id} \rightarrow \mb{R}^{\featDim} \times \mb{R}^4$. 
The backbone $\backboneFunc_{\detParam}: \mb{X} \rightarrow \mb{R}^{\featDim} \times \mb{R}^4$ predicts the location $\bb{b}_i$ of the objects and extracts its latent features $\featVar_i$, followed by a classifier for class prediction $\clsFunc_\detParam: \mb{R}^\featDim \rightarrow \mb{Y}$.
Our goal is to enable the object detector to identify objects drawn from an unknown distribution $\mb{P}_{ood}$ -- \gls{ood} objects. %with an module $\oodFunc: \mb{R}^\featDim \rightarrow \{0, 1\}$ that can predict $0$ for features $\pb{\featVar}$ of $\{ \pb{x}$, $\pb{b} \}$ drawn from some unknown distribution $\mb{P}_{ood}$ different to $\mb{P}_{id}$ and $1$ for those drawn from $\mb{P}_{id}  $\mb{P}_{ood}$$.
A promising way \textit{without collecting training data for \gls{ood} objects} is to realize with a density estimator, e.g. \gls{nf} in this work. 
This density estimator identifies \gls{ood} objects with low likelihoods after being trained \textit{only} on data drawn from $\mb{P}_{id}$. 
Driven by semantic richness and efficiency of representations learned on the logit space (pre-softmax layer)~\cite{wei2022logitnorm, miller2021uncertainty}, we select the logits as the features $\featVar$ in this work, i.e. $d=C$, but the proposed method is ready to generalize to high-dimensional latent features.  
% We assume that there is no overlapping between $\mb{P}_{id}$ and $\mb{P}_{ood}$ so that \gls{ood} detection is easier to learn~\cite{fang2022out}.

% \subsection{Preliminaries}
% Before introducing the main idea, we briefly provide the preliminaries of the core building blocks, i.e. Normalizing Flows and the Information Bottleneck objective in the following, which are of advantage to understand the proposed method.

\subsection{Toplogical Mismatch in Normalizing Flows -- And How to Solve It}
\label{tp_problem}

\iffalse
\begin{wrapfigure}[12]{r}{0.475\textwidth}
   \centering
   \vspace{-25pt}
   %
   \subfloat[\(p(\featVar)\)\label{fig:filaments:a}]{\includegraphics[width=0.33\linewidth]{materials/filament/moons_gauss_contour_target.png}}
   \hfill
   \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\)\label{fig:filaments:b}]{\includegraphics[width=0.33\linewidth]{materials/filament/moons_gauss_contour_model.png}}
   \hfill
   \subfloat[\(p(\baseVar)\)\label{fig:filaments:c}]{\includegraphics[width=0.33\linewidth]{materials/filament/moons_gauss_contour_base.png}}
   %
   \caption{Filament connect modes in the modeled distribution (b) if using uni-modal base (c) to model multi-modal distribution (a). Reproduction of Figure 1 in \citep{stimper2022resampling}.}
   \label{fig:filaments}
\end{wrapfigure}
\fi
\begin{wrapfigure}[20]{r}{0.55\textwidth}
   \centering
   \vspace{-25pt}
   %
   \subfloat[\(p(\featVar|y=0)\)\label{fig:filaments:a}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_gt_density_0.png}}
   \hfill
   \subfloat[\(p_{\flowParam, \baseParam}(\featVar|y=0)\)\label{fig:filaments:b}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_gmm_cls_wib_density_0.png}}
   \hfill
   \subfloat[\(p_{\baseParam}(\baseVar|y=0)\)\label{fig:filaments:c}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_gmm_cls_wib_base_0.png}}
   %
   \\
   %
   \subfloat[\(p(\featVar|y=0)\)\label{fig:filaments:a}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_gt_density_0.png}}
   \hfill
   \subfloat[\(p_{\flowParam, \baseParam}(\featVar|y=0)\)\label{fig:filaments:b}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_resampled_cls_out_wib_density_0.png}}
   \hfill
   \subfloat[\(p_{\baseParam}(\baseVar|y=0)\)\label{fig:filaments:c}]{\includegraphics[width=0.33\linewidth]{materials/toy/moons_resampled_cls_out_wib_base_0.png}}
   \caption{Filament connect modes in the modeled class-conditional distribution (b) if using (trainable) uni-modal base (c) for the multi-modal target (a).}
   \label{fig:filaments}
\end{wrapfigure}
%
\gls{nf} are known to be universal distribution approximators~\cite{papamakarios2021normalizing}. That is, they can model any complex target distribution $p(\featVar)$ on a space $\mb{R}^\featDim$ by defining $\featVar$ as a transformation $\flowFunc_\flowParam: \mb{R}^\featDim \rightarrow \mb{R}^\featDim$ parameterized by $\flowParam$ from a well-defined base distribution $p_{\baseParam}(\baseVar)$ parameterized by $\baseParam$: 
\begin{equation}
    \label{flowGeneration}
    \featVar = \flowFunc_\flowParam(\baseVar) \text{~~where~~} \baseVar \sim p_{\baseParam}(\baseVar)\,,
\end{equation}
where $\baseVar \in \mb{R}^\featDim$ and $p_{\baseParam}$ is commonly chosen as a uni-modal Gaussian.
By designing $T_{\flowParam}$ to be a \textit{diffeomorphism}, that is, a bijection where both $T_{\flowParam}$ and $T^{-1}_{\flowParam}$ are differentiable. We can compute the likelihood of the input $\featVar$ exactly based on the change-of-variables formula~\cite{bogachev2007measure}: 
\begin{equation}
    \label{pdf_computation}
    p(\featVar) =  p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar))|\det(J_{T_{\flowParam}^{-1}}(\featVar))|\,,
\end{equation}
where $J_{T_{\flowParam}^{-1}}(\featVar) \in \mb{R}^{\featDim \times \featDim}$ is the Jacobian of the inverse $\flowFunc_{\flowParam}^{-1}$ with respect to $\featVar$.
% The transformation $\flowFunc_\flowParam$ can constructed by composing a series of bijective maps denoted by $\subflowFunc_{\flowParam}^i$ 
%\flowFunc_\oodParam = \subflowFunc_1 \circ \subflowFunc_2 \circ ...  \circ \subflowFunc_\flowNum$.
When the target distribution is unknown but samples thereof are available, we can estimate the parameter $(\phi, \psi)$ by minimizing the forward \gls{kld}, which is equivalent to maximizing the expected \gls{ll} over the samples.
% \def\Jdet{|\det(J_{T_{\flowParam}^{-1}}(\featVar))|}
% \def\baseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar)))}
% \begin{equation}
%     \label{mle}
%     \text{LL}(\flowParam, \baseParam) = \mathbb{E}_{p(\featVar)}\left[ \log \baseL + \log \Jdet \right]
% \end{equation}

% \paragraph{Topological Problems of \gls{nf}} % TODO: 
% \todo{explain this with the toy classification visualization}
\paragraph{Topological Mismatch}
However, since the base distribution $p_\baseParam(\baseVar)$ is usually a uni-modal Gaussian and $\flowFunc_\flowParam$ is a diffeomorphism, problems arise for modeling data distribution with different topological properties. These include well-separated multi-modal distributions or distributions with disconnected components. For example, in \Cref{fig:density_toy:d} and \Cref{fig:density_toy:f}, one can see that this leads to density filaments between the modes, i.e. two arcs in this case. \citet{cornish2020relaxing} have shown that flows require a bijection with infinite \textit{bi-Lipshitz constant} if modeling a target distribution with disconnected support using a unimodal base distribution. Importantly, an infinite bi-Lipshitz renders the bijection to be numerically "non-invertible", thus, causing optimization instability and unreliability during training.


\paragraph{How to Solve It} One practical mitigation is by enriching the expressiveness of the flows. For example, by (a) increasing number of layers or parameters, (b) using more complex base distributions, or (c) employing multiple \gls{nf}. It is important to note that especially (a) and (c) could escalate the computational cost and memory burden, which is unfavorable for robotic systems commonly with restricted computing resources. Moreover, scaling the normalizing flow's expressivity, (a) or (c), comes with less guarantee on stabilizing the optimization~\cite{hagemann2021stabilizing} and securing the likelihood calculation. For this reason, we pursue (b) and attempt to compensate for the complexity of the transformation with the elasticity of the base distribution. In other words, we use a more flexible but efficient base distribution to trade off a costly but sufficiently expressive bijection of the normalizing flow. This way we aim to capture desirable topological properties of the target distribution~\cite{jaini2020tails}.

Following prior work~\cite{fetaya2019understanding}, we use a class-conditional base distribution. This way we get similar benefits like combining multiple flows (c), however, without having to burden the computational cost. Even though a class-conditional distribution can specialize on a smaller fraction of the dataset containing similar instances, in real-world applications, it will surely manifest in a multi-modal distribution. We introduce the learnable class-conditional distribution, called Conditional Resampled Base Distributions, in \Cref{crsb}, which is capable of approximating complex distributions and thus more accurately capturing their topological properties.

% \begin{wrapfigure}[50]{r}{1.0\textwidth}
\begin{figure}
    \centering
    \vspace{-15pt}
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.2\linewidth]{materials/toy/moons_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.2\linewidth]{materials/toy/moons_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:j}]{\includegraphics[width=0.2\linewidth]{materials/toy/moons_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.2\linewidth]{materials/toy/moons_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.2\linewidth]{materials/toy/moons_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:a}]
    {\includegraphics[width=0.2\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:b}]
    {\includegraphics[width=0.2\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.2\linewidth]{materials/toy/rings_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.2\linewidth]{materials/toy/rings_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.2\linewidth]{materials/toy/rings_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.2\linewidth]{materials/toy/circle_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.2\linewidth]{materials/toy/circle_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:j}]{\includegraphics[width=0.2\linewidth]{materials/toy/circle_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.2\linewidth]{materials/toy/circle_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.2\linewidth]{materials/toy/circle_resampled_cls_out_wib_density.png}}
    %
    \caption{Class conditional densities plotted in \([-3,3]^2\) using RealNVP bijection with class conditional MoG, where each class is modeled by a unimodal Gaussian%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , and cRSB. We use 4 layers with cRSB and 5 layers with MoG to balance the compute of acceptance rate \(a_{\baseParam}\).
    \todo{Simon-remove space between rows, replace MoG w/o IB and cRSB w/o IB with base distribution visualization.}}
    \label{fig:density_toy}
\end{figure}
% \end{wrapfigure}
%
Unfortunately, directly training \gls{nf} with a conditional base distribution can lead to underperformance as observed in preliminary experiments and reported by~\citet{fetaya2019understanding}.
This attributes to the lack of explicit control for the balance between generative and discriminative modeling in the likelihood-based training objective of \gls{nf}.
To alleviate this, we train the normalizing flow with class-conditional base distribution using the so-called Information Bottle-neck objective (see \Cref{sec:ib}). Intuitively, the Information Bottleneck minmizes the mutual information between the base distribution \(p(\baseVar)\) and the distribution in the latent space \(p(\featVar)\), while maximizing the mutual information between base distribution \(p(\baseVar)\) and the target variable \(p(y)\).

\iffalse
\subsubsection{Conditional Resampled Base Distributions}
\label{crsb}
\begin{figure}
    \centering
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:a}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:b}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:c}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:e}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:i}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:k}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:i}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:k}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_density.png}}
    %
    \caption{Class conditional densities plotted in \([-3,3]^2\) using RealNVP bijection with class conditional MoG, where each class is modeled by a unimodal Gaussian%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , and cRSB. We use 4 layers with cRSB and 5 layers with MoG to balance the compute of acceptance rate \(a_{\baseParam}\).  We train with regular KL divergence and IB objective.
    \todo{Simon-remove space between rows, replace MoG w/o IB and cRSB w/o IB with base distribution visualization.}}
    \label{fig:density_toy}
\end{figure}

\begin{figure}
    \centering
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:a}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:b}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=0)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_base_0.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=1)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_base_1.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=0)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_base_0.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=1)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_base_1.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=0)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_base_0.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar|y=1)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_base_1.png}}
    %
    \caption{Class conditional densities plotted in \([-3,3]^2\) using RealNVP bijection with class conditional MoG, where each class is modeled by a unimodal Gaussian%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , and cRSB. We use 4 layers with cRSB and 5 layers with MoG to balance the compute of acceptance rate \(a_{\baseParam}\).
    \todo{Simon-remove space between rows, replace MoG w/o IB and cRSB w/o IB with base distribution visualization.}}
    \label{fig:density_toy}
\end{figure}


\begin{figure}
    \centering
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:a}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:b}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_wib_base.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_base.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_wib_base.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_base.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_1.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_wib_base.png}}
    %
    \subfloat[\(p_{\flowParam, \baseParam}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_density.png}}
    %
    \subfloat[\(p_{\baseParam}(\baseVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_base.png}}
    %
    \caption{Class conditional densities plotted in \([-3,3]^2\) using RealNVP bijection with class conditional MoG, where each class is modeled by a unimodal Gaussian%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , and cRSB. We use 4 layers with cRSB and 5 layers with MoG to balance the compute of acceptance rate \(a_{\baseParam}\).
    \todo{Simon-remove space between rows, replace MoG w/o IB and cRSB w/o IB with base distribution visualization.}}
    \label{fig:density_toy}
\end{figure}
\fi

We propose to capture the complex topological properties in the target distribution with a more expressive base distribution instead of the uni-model Gaussian. 
To the end, we introduce \gls{crsb} by extending a powerful unconditional base distribution \gls{rsb}~\cite{stimper2022resampling} to support class-conditional modeling.
The idea of \gls{rsb} is to replace the uni-modal Gaussian with a learnable distribution that can approximate a complex distribution based on \gls{lars}~\cite{bauer2019resampled}. 
\gls{lars} iteratively re-weighs samples drawn a proposal distribution $\pi(\baseVar)$, e.g. a standard Gaussian, through a learned acceptance function $a_{\baseParam}: \mathcal{R}^{\featDim} \rightarrow [0,1]$.
To reduce the computation cost in practice, this process is truncated by accepting the $T$-th samples if the previous $T-1$ samples get rejected. 
% The resulting distribution is as follows:
% \begin{equation}
%     \label{rsb_base}
%     p_{\baseParam}(\baseVar) = (1 - \alpha_T)\frac{a_{\baseParam}(\baseVar)\pi(\baseVar)}{Z} + \alpha_T\pi(\baseVar)
% \end{equation}, 
To take into account conditional information, we need to conditionalize the learnable acceptance function $a_{\baseParam}(\baseVar)$ by modifying the output dimension of the acceptance function  $a_{\baseParam}(\baseVar)$ to predict the acceptance rate for each class. 
With this extension, we have the following conditional base distribution:
\begin{equation}
    \label{rsb_base}
    p_{\baseParam}(\baseVar|y=k) = (1 - \alpha_T)\frac{a_{\baseParam}(\baseVar)\pi(\baseVar|y_k)}{Z_k} + \alpha_T\pi(\baseVar),
\end{equation} 
where $a_{\baseParam}: \mathcal{R}^{\featDim} \rightarrow [0,1]^{C}$ and $\alpha_T = (1-Z)^{T-1}$, where Z is the normalization factor for $\pi(\baseVar)a_{\baseParam}(\baseVar)$, which can be estimated via Monte Carlo Sampling.
\paragraph{Discussion} There is another way to conditionalize the acceptance function by making the input $\baseVar$ conditioning on the class.  
However, this way requires higher computation overhead, i.e. multiple forward passes for each class when we need a marginalized base density for \gls{ood} detection (see sub-sec. \ref{inference}) without much performance gain observed in preliminary experiments.
On the other hand, inspired by the \gls{gm}, we also tested class conditional Gaussians for the proposal distribution $\pi(\baseVar)$.
However, the hypothesized expressiveness did not transfer to performance increase in preliminary experiments, we leave the investigation of this as future work. \todo{Jianxiang-adding discussion of conditional MoG could not fix multi-modal with only one Gaussian}

% \subsubsection{\gls{ib} for conditional \gls{nf}}
% Class conditional information is valuable for accurate density estimation of data with semantic class labels e.g. $p(\featVar|\bb{y})$.
\subsubsection{Training with Information Bottleneck}\label{sec:ib}

\begin{wrapfigure}[18]{r}{0.35\textwidth}
  \centering
  \vspace{-25pt}
  %
  \subfloat[\(y=0\), w/o IB\label{fig:rings_crsb_acceptance:a}]{\includegraphics[width=0.49\linewidth]{materials/toy/moons_resampled_cls_out_woib_a_0.png}}
  \hfill
  \subfloat[\(y=1\), w/o IB\label{fig:rings_crsb_acceptance:b}]{\includegraphics[width=0.49\linewidth]{materials/toy/moons_resampled_cls_out_woib_a_1.png}}
  %
  \\
  %
  \subfloat[\(y=0\), w/ IB\label{fig:rings_crsb_acceptance:a}]{\includegraphics[width=0.49\linewidth]{materials/toy/moons_resampled_cls_out_wib_a_0.png}}
  \hfill
  \subfloat[\(y=1\), w/ IB\label{fig:rings_crsb_acceptance:b}]{\includegraphics[width=0.49\linewidth]{materials/toy/moons_resampled_cls_out_wib_a_1.png}}
  %
  \caption{Acceptance rate \(a_{\baseParam}(\baseVar)\) after training cRSB w/o and w/ IB for class-conditional ``moons''.}
  \label{fig:rings_crsb_acceptance}
\end{wrapfigure}
%
\gls{ib} provides a principle and explicit way to coordinate the influences from two different variables, e.g. $\featVarCap$ and $Y$ for learning the latent variable $\baseVarCap$.
\gls{ib}~\cite{tishby2000information} is an information theoretic approach for extracting relevant information measured by \gls{mi} about one variable $Y$ from another one $\featVarCap$.
This relevant information is squeezed through a 'bottleneck' of the information flow between $\featVarCap$ and $Y$ in form of another latent variable $\baseVarCap$.
Therefore, \gls{ib} strives to minimize the \gls{mi} $I(\featVarCap, \baseVarCap)$ between $\featVarCap$ and $\baseVarCap$ and simultaneously maximize the \gls{mi} $I(\baseVarCap, Y)$ between $\baseVarCap$ and $Y$ with a trade-off parameter to balance the two aspects.
% \begin{equation}
%     \label{ib}
%     \mathcal{L}_{IB} = I(\featVarCap, \baseVarCap) - \beta I(\baseVarCap, Y) 
% \end{equation}.

However, \gls{ib} is not directly ready for adoption as it is problematic to estimate the \gls{mi} between the input variable $\featVarCap$ and the latent $\baseVarCap$ of a flow due to the deterministic and bijective mapping $\flowFunc_\flowParam$, which raises the issue of invalidity of the definition of joint distribution between $\featVarCap$ and $\baseVarCap$.
 To this end, we adopt a technique proposed by~\citet{ardizzone2020training} which injects a small amount of noise $\epsilon$ into the input $\featVarCap$ for valid density definition and introduces an asymptotically exact version of \gls{ib} by defining another function $\hat{I}(\cdot, \cdot)$ to measure the relevant information between two random variables (more details in appendix):
\def\IBJdet{|\det(J_{T_{\flowParam}^{-1}}(\featVar+\epsilon))|}
\def\IBbaseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)))}
\def\condIBbaseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)|y))}
\def\SumCondIBbaseL{\sum_{y\prime}(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)|y\prime))}
\begin{equation}
    \label{ib_nf}
    \mathcal{L}_{\text{IBNF}} =  \hat{I}(\featVarCap, \baseVarCap) - \beta \hat{I} (\baseVarCap, Y)  % \text{~~~~with}
\end{equation}
\begin{equation}
    \label{ci_yz}
     \hat{I}(\baseVarCap, Y) = \mathbb{E}_{p(y)}\left[ \log \frac{p_{\baseParam}(\baseVar|y)p(y)}{\sum_{y\prime}(p_{\baseParam}(\baseVar|y\prime)p(y\prime))} \right]  % \text{~~~~and} 
\end{equation}
\begin{equation}
    \label{ci_xz}
    \hat{I}(\featVarCap, \baseVarCap)=\mathbb{E}_{p(\featVar), p(\epsilon)}\left[ - \log {\sum_{y\prime}(p_{\baseParam}(\baseVar|y\prime))} - \log \IBJdet \right],
\end{equation}
where $\baseVar=\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)$ and $p(\epsilon) = \mathcal{N}(0, \sigma^2 \mathcal{I}_{\featDim})$ is a zero-meaned Gaussian with variance $\sigma^2$.
$\beta$ is a trade-off parameter to balance the two aspects.
With the flexible conditional base distributions defined in Eq. \ref{rsb_base}, we can train \textit{topologically matched} \gls{nf} with \gls{ib} by substituting \gls{crsb} into the conditional base probability $p_{\flowParam}(\baseVar|y)$ in Eq. \ref{ci_yz}.
More noteworthy, we observed that the \gls{ib} is able to regularize the acceptance rate learning for \gls{crsb} to better assimilate the topological structure of the target distribution, leading to an overall improved performance on accurately approximating the complex target distribution ( see \Cref{fig:rings_crsb_acceptance}). 

\subsection{Detecting OOD Objects}
\label{inference}
During test time, we detect the \gls{ood} objects based on the \glsfirst{ll} estimated from the topologically matched \gls{nf} trained with \gls{ib} as described in previous sub-sections.
% For evaluation, to sidestep the influences of various selected thresholds, we measure the performance with \gls{auroc}. 
We marginalize over classes for the base distribution defined in Eq. \ref{rsb_base} and compute the final \gls{ll} based on the Change-of-Variables formula given the logits $\pb{\featVar}$ from the image and the object bounding box $\{ \pb{x}$, $\pb{b} \}$:
\begin{equation}
    \label{test_ll}
    \operatorname{LL}_{test}(\pb{\featVar})=\log {\sum_{y\prime}(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\pb{\featVar})|y\prime))} - \log |\det(J_{T_{\flowParam}^{-1}}(\pb{\featVar}))|.
\end{equation}
As we model the complicated \gls{id} with \gls{nf}, the expected \gls{ll} for \gls{id} objects should be higher than \gls{ood} ones. 
A threshold to distinguish \gls{id} and \gls{ood} objects can be estimated from the training set. 

==> main/simons_trash.tex <==
\subsubsection{Conditional Resampled Base Distributions}
\label{crsb}
\begin{figure}
    \centering
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:a}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:b}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:c}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:d}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_gmm_cls_wib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:e}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:f}]
    {\includegraphics[width=0.165\linewidth]{materials/toy/rings_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gt_density_1.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:i}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_gmm_cls_wib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:k}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/circle_resampled_cls_out_wib_density.png}}
    %
    \\
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:density_toy:g}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:density_toy:h}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gt_density_1.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/o IB\label{fig:density_toy:i}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/ IB\label{fig:density_toy:j}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_gmm_cls_wib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/o IB\label{fig:density_toy:k}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/ IB\label{fig:density_toy:l}]{\includegraphics[width=0.165\linewidth]{materials/toy/moons_resampled_cls_out_wib_density.png}}
    %
    \caption{Class conditional density estimation using identically configured bijections but with two different base distributions, i.e. class conditional MoG, where each class is modeled by a unimodal Gaussian%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , and cRSB trained with regular KL divergence and IB objective.
    \todo{Simon-remove space between rows, replace MoG w/o IB and cRSB w/o IB with base distribution visualization.}}
    \label{fig:density_toy}
\end{figure}



\begin{figure}
    \centering
    %
    \subfloat[Ground truth\label{fig:rings_density:a}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_gt_density.png}}
    %
    \subfloat[c\(\mathcal{N}\) w/o IB\label{fig:rings_density:b}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_gmm_woib_density.png}}
    %
    \subfloat[c\(\mathcal{N}\) w/ IB\label{fig:rings_density:c}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_gmm_wib_density.png}}
    %
    \subfloat[cRSB w/o IB\label{fig:rings_density:d}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_woib_density.png}}
    %
    \subfloat[cRSB w/ IB\label{fig:rings_density:e}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_wib_density.png}}
    %
    \\
    %
    \subfloat[Ground truth\label{fig:rings_density:f}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_gt_test_samples_cls.pdf}}
    %
    \subfloat[c\(\mathcal{N}\) w/o IB\label{fig:rings_density:g}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_gmm_woib_test_samples_cls.pdf}}
    %
    \subfloat[c\(\mathcal{N}\) w/ IB\label{fig:rings_density:h}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_gmm_wib_test_samples_cls.pdf}}
    %
    \subfloat[cRSB w/o IB\label{fig:rings_density:i}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_woib_test_samples_cls.pdf}}
    %
    \subfloat[cRSB w/ IB\label{fig:rings_density:j}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_wib_test_samples_cls.pdf}}
    %
    \caption{Class conditional density estimation using identically configured bijections with class conditional Gaussian c\(\mathcal{N}\), defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\), or cRSB base distribution and regular KL divergence and IB objective. The first row visualizes the density \(p(\featVar)\) and the second the predicted classes for \(\arg\max_{c}p(\featVar|y = c)p(y = c)\).}
    \label{fig:rings_density}
\end{figure}


\begin{figure}
    \centering
    %
    \subfloat[Ground truth\label{fig:rings_density:f}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_gt_test_samples_cls.pdf}}
    %
    \subfloat[Ground truth\label{fig:rings_density:a}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_gt_density.png}}
    %
    \subfloat[c\(\mathcal{N}\) w/o IB\label{fig:rings_density:b}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_model_gmm_woib_density.png}}
    %
    \subfloat[c\(\mathcal{N}\) w/ IB\label{fig:rings_density:h}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_model_gmm_wib_density.png}}
    %
    \subfloat[cRSB w/o IB\label{fig:rings_density:d}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_model_woib_density.png}}
    %
    \subfloat[cRSB w/ IB\label{fig:rings_density:e}]{\includegraphics[width=0.155\linewidth]{materials/toy/rings_model_wib_density.png}}
    %
    \caption{Class conditional density estimation using identically configured bijections with class conditional Gaussian c\(\mathcal{N}\), defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\), or cRSB base distribution and regular KL divergence and IB objective. The first row visualizes the density \(p(\featVar)\) and the second the predicted classes for \(\arg\max_{c}p(\featVar|y = c)p(y = c)\).}
    \label{fig:rings_density}
\end{figure}


\begin{figure}
    \centering
    %
    \begin{minipage}[t]{.795\linewidth}
    \subfloat[Ground truth\label{fig:rings_density:a}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_gt_density.png}}
    %
    \subfloat[c\(\mathcal{N}\) w/o IB\label{fig:rings_density:b}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_gmm_woib_density.png}}
    %
    \subfloat[cRSB w/o IB\label{fig:rings_density:d}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_woib_density.png}}
    %
    \subfloat[cRSB w/ IB\label{fig:rings_density:e}]{\includegraphics[width=0.195\linewidth]{materials/toy/rings_model_wib_density.png}}
    \end{minipage}
    %
    \begin{minipage}[t]{.195\linewidth}
        \includegraphics[width=0.48\linewidth]{materials/toy/rings_gt_test_samples_cls.pdf}
        %
        \includegraphics[width=0.48\linewidth]{materials/toy/rings_model_gmm_woib_test_samples_cls.pdf}
        \\
        \includegraphics[width=0.48\linewidth]{materials/toy/rings_model_woib_test_samples_cls.pdf}
        %
        \includegraphics[width=0.48\linewidth]{materials/toy/rings_model_wib_test_samples_cls.pdf}
    \end{minipage}
    \caption{Class conditional density estimation using identically configured bijections with class conditional Gaussian c\(\mathcal{N}\), defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\), or cRSB base distribution and regular KL divergence and IB objective. The first row visualizes the density \(p(\featVar)\) and the second the predicted classes for \(\arg\max_{c}p(\featVar|y = c)p(y = c)\).}
    \label{fig:rings_density}
\end{figure}




\section{Methods}
\label{methods}
We start with the problem formulation of \gls{ood} detection in the context of Open-Set Object Detection~\cite{miller2021uncertainty, Dhamija_2020_WACV}, which is more relevant to real-world robotic perception~\cite{lee2022virtual, feng2022bayesian}.
The goal is to train an object detector that can not only localize and categorize the known objects seen during training but also \textit{identify unknown objects} unseen during training but falsely detected during test-time.
This is more challenging than image classification due to the fine-grained reasoning on object-level instead of image-level and the necessary requirement of real-time inference, which is meanwhile beneficial for robots in need of timely decision-making. 
We aim to achieve such object detector with a topologically matched \gls{nf} trained with \gls{ib} due to several appealing properties of \gls{nf} such as its easy compatibility with existing models and the fast inference with only single forward pass.
In the following, we will first introduce the problem, briefly describe the fundamental topological constraint of \gls{nf} and elaborate how we employ expressive base distributions to mitigate this problem.

\paragraph{Problem Formulation} 
\def\flowNum{n}
\def\baseParam{\psi}
\def\baseVarCap{Z}
\def\baseVar{\bb{z}}
\def\flowFunc{T}
\def\subflowFunc{t}
\def\flowParam{\phi}
\def\oodFunc{h}
\def\featDim{d} 
\def\featVarCap{U}
\def\featVar{\bb{u}}
\def\detFunc{F} 
\def\detParam{\theta} 
\def\backboneFunc{f} 
\def\clsFunc{g}
We define a data-set $\mathcal{D}_{id}=\{ (\bb{x}_i, \bb{b}_i, y_i) \}_{i=1}^{N}$ consisting of $N$ samples of objects with corresponding object bounding box coordinates $\bb{b}_i \in \mb{R}^4$ and class label $y_i \in \mb{Y} = \{1,2,...,C\}$ on an image $\bb{x}_i \in \mb{X}_{id}$ drawn from some known distribution $\mb{P}_{id}=\mb{X}_{id} \times \mb{Y} \times \mb{R}^4$. 
We then use it to train an object detector $\detFunc_\detParam = \backboneFunc_\detParam \circ \clsFunc_\detParam$ parameterized by $\detParam$, where there is one module for both bounding box prediction and feature extraction $\backboneFunc_{\detParam}: \mb{X}_{id} \rightarrow \mb{R}^{\featDim} \times \mb{R}^4$. 
Another one is a classifier for class prediction $\clsFunc_\detParam: \mb{R}^\featDim \rightarrow \mb{Y}$ for each predicted bounding box.
Our goal is to equip the object detector with an module $\oodFunc: \mb{R}^\featDim \rightarrow \{0, 1\}$ that can predict $0$ for features $\pb{\featVar}$ of $\{ \pb{x}$, $\pb{b} \}$ drawn from some unknown distribution $\mb{P}_{ood}$ different to $\mb{P}_{id}$ and $1$ for those drawn from $\mb{P}_{id}$.
A promising way with no effort on collecting data from $\mb{P}_{ood}$ is to realize $\oodFunc$ with a density estimator, e.g. \gls{nf} in this work. 
This density estimator identifies data from $\mb{P}_{ood}$ with low likelihoods after being trained \textit{only} on data drawn from $\mb{P}_{id}$. 
Inspired by semantic and efficient representations learned on the logit space (pre-softmax layer)~\cite{wei2022logitnorm, miller2021uncertainty}, we select the logits output from $\clsFunc_\detParam$ as the feature $\featVar$ used in this work, i.e. $d=C$.  
% We assume that there is no overlapping between $\mb{P}_{id}$ and $\mb{P}_{ood}$ so that \gls{ood} detection is easier to learn~\cite{fang2022out}.

% \subsection{Preliminaries}
% Before introducing the main idea, we briefly provide the preliminaries of the core building blocks, i.e. Normalizing Flows and the Information Bottleneck objective in the following, which are of advantage to understand the proposed method.

\subsection{Toplogical Mismatch in Noramlizing Flows}
\label{tp_problem}
\begin{figure}
    \centering
    %
    \subfloat[\(p(\featVar|y = 0)\), ground truth\label{fig:rings_density:a}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_0.png}}
    %
    \subfloat[\(p(\featVar|y = 1)\), ground truth\label{fig:rings_density:b}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_gt_density_1.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/o IB\label{fig:rings_density:c}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_model_gmm_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\MoG w/ IB\label{fig:rings_density:d}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_model_gmm_wib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/o IB\label{fig:rings_density:e}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_model_woib_density.png}}
    %
    \subfloat[\(\tilde{p}(\featVar)\),\\cRSB w/ IB\label{fig:rings_density:f}]{\includegraphics[width=0.165\linewidth]{materials/toy/rings_model_wib_density.png}}
    %
    \caption{Class conditional density estimation using identically configured bijections with class conditional MoG%, defined as \(\mathcal{N}(\boldsymbol{\mu}_c, \boldsymbol{\Sigma}_c)\)
    , or cRSB base distribution and regular KL divergence and IB objective. The first row visualizes the density \(p(\featVar)\) and the second the predicted classes for \(\arg\max_{c}p(\featVar|y = c)p(y = c)\).}
    \label{fig:rings_density}
\end{figure}


\gls{nf} provide an expressive way to model complex target distribution $p(\featVar)$ on a space $\mb{R}^\featDim$ by defining $\featVar$ as a transformation $\flowFunc_\flowParam: \mb{R}^\featDim \rightarrow \mb{R}^\featDim$ parameterized by $\flowParam$ from a well-defined base distribution $p_{\baseParam}(\baseVar)$ parameterized by $\baseParam$: 
\begin{equation}
    \label{flowGeneration}
    \featVar = \flowFunc_\flowParam(\baseVar) \text{~~where~~} \baseVar \sim p_{\baseParam}(\baseVar),
\end{equation}
where $\baseVar \in \mb{R}^\featDim$ and $p_{\baseParam}$ is commonly chosen as a uni-modal Gaussian.
By designing $T_{\flowParam}$ to be a \textit{diffeomorphism}, that is, it needs to be \textit{invertible} and both $T_{\flowParam}$ and $T^{-1}_{\flowParam}$ must be \textit{differentiable}, we can compute the likelihood of the input $\featVar$ exactly based on the change-of-variables formula~\cite{bogachev2007measure}: 
\begin{equation}
    \label{pdf_computation}
    p_{\featVarCap}(\featVar) =  p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar))|\det(J_{T_{\flowParam}^{-1}}(\featVar))|,
\end{equation}
where $J_{T_{\flowParam}^{-1}}(\featVar) \in \mb{R}^{\featDim \times \featDim}$ is the Jacobian of the inverse $\flowFunc_{\flowParam}^{-1}$ with respect to $\featVar$.
% The transformation $\flowFunc_\flowParam$ can constructed by composing a series of bijective maps denoted by $\subflowFunc_{\flowParam}^i$ 
%\flowFunc_\oodParam = \subflowFunc_1 \circ \subflowFunc_2 \circ ...  \circ \subflowFunc_\flowNum$.
When the target distribution is unknown but samples thereof are available, we can estimate the parameter $(\phi, \psi)$ by minimizing the forward \gls{kld}, which is equivalent to maximizing the expected \gls{ll} over the samples.
% \def\Jdet{|\det(J_{T_{\flowParam}^{-1}}(\featVar))|}
% \def\baseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar)))}
% \begin{equation}
%     \label{mle}
%     \text{LL}(\flowParam, \baseParam) = \mathbb{E}_{p(\featVar)}\left[ \log \baseL + \log \Jdet \right]
% \end{equation}

% \paragraph{Topological Problems of \gls{nf}} % TODO: 
% \todo{explain this with the toy classification visualization}
However, by definition, $\flowFunc_\flowParam$ is a diffeomorphism and the base distribution $p_\baseParam(\baseVar)$ is usually a uni-modal Gaussian.
This raises a problem for modeling data distribution with different topological properties, e.g. well-separated multi-model distributions, distributions with disconnected components, which seems critical for data hypothesized to follow a clustering structure e.g. the data with different class labels.
For example, in Fig \ref{tp_problem}, the MoG with one uni-modal gaussian per class stuggles to recover the target distribution with two modes.
As proofed by~\citet{cornish2020relaxing}, flows that can recover the target distribution perfectly need to have infinite \textit{bi-Lipshitz constant} which would make the flows numerically "non-invertible", causing optimization instability and unreliability on computing the exact \glsfirst{ll}~\cite{behrmann2021understanding}, which might be destructive when applying \gls{nf} for \gls{ood} detection.   
One way to mitigate this is by enriching the expressiveness of flows such as increasing depth (e.g. number of layers) or width (e.g. mixtures of flow), but this could escalate the computational cost and memory burden, which is unfavorable for robotic systems commonly with restricted computing resources.
As this limitation is affected by both the transformation and the base distribution, there is a \textit{trade-off} between a flexible base distribution and an expressive transform to capture desirable topological properties of the target distribution~\cite{jaini2020tails}.
We attempt to compensate the complexity of the transformation with elasticity of the base distribution, that might be beneficial for diverse types of flow architectures.
% In the following, we introduce one kind of these flexible base distributions on which our work is based.


\subsection{Topologically Matched Normalizing Flows with Information Bottleneck}
%
\begin{wrapfigure}[17]{r}{0.35\textwidth}
  \centering
  \vspace{-15pt}
  %
  \subfloat[\(y=0\), w/o IB\label{fig:rings_crsb_acceptance:a}]{\includegraphics[width=0.49\linewidth]{materials/toy/rings_model_woib_0_a.png}}
  \hfill
  \subfloat[\(y=1\), w/o IB\label{fig:rings_crsb_acceptance:b}]{\includegraphics[width=0.49\linewidth]{materials/toy/rings_model_woib_1_a.png}}
  %
  \\
  %
  \subfloat[\(y=0\), w/ IB\label{fig:rings_crsb_acceptance:a}]{\includegraphics[width=0.49\linewidth]{materials/toy/rings_model_wib_0_a.png}}
  \hfill
  \subfloat[\(y=1\), w/ IB\label{fig:rings_crsb_acceptance:b}]{\includegraphics[width=0.49\linewidth]{materials/toy/rings_model_wib_1_a.png}}
  %
  \caption{Acceptance rate \(a_{\baseParam}(\baseVar)\) after training cRSB w/o and w/ IB.}
  \label{fig:rings_crsb_acceptance}
\end{wrapfigure}
%
As mentioned above, the topological mismatch can lead to diminishing performance and numerical instability of applying \gls{nf}. 
The straightforward solutions such as adding more layers or employing mixtures of flows can lead to high computation and memory demands with less guarantee on stabilizing the optimization~\cite{hagemann2021stabilizing} and securing the likelihood calculation. 
To mitigate this issue, in this work, we shift the focus to the other end of the spectrum, that is, to increase the expressiveness of the base distribution, hence making it closer to the target distribution.
Moreover, to further leverage class information in object detection for more effective \gls{ood} detection, we train our toplogically matched \gls{nf} with \gls{ib}.

% To this end, we suggest two more expressive conditional base distributions, the first one is the well-known \glsfirst{gm}:
% \begin{equation}
%     \label{gm_base}
%     p_{\baseParam}(\baseVar|y=k) =  \mathcal{N}(\baseVar|\mu_k, \Sigma_k)
% \end{equation}, 
% where $\baseParam=\{(\mu_k, \Sigma_k)\}_{k=1}^{C}$. 
% \gls{gm} is a popular choice for a multi-modal base distribution for \gls{nf} besides the uni-modal Gaussian.
% Although \gls{gm} is highly flexible in theory, it is non-trivial to obtain an optimal model through the traditional \gls{em} algorithm~\cite{izmailov2020semi}. 
% In practice, it is empirically better to initialize the means of different Gaussians far enough to each other and freeze them, leading to a base distribution with topology of multiple modes.
% This hampers the actual modeling capacity of \gls{gm} for approximating complex distributions.

\subsubsection{Conditional Resampled Base Distributions}
\label{crsb}

We propose to capture the complex topological properties in the target distribution with a more expressive base distribution instead of the uni-model Gaussian. 
To the end, we introduce \gls{crsb} by extending a powerful unconditional base distribution \gls{rsb}~\cite{stimper2022resampling} to support class-conditional modeling.
The idea of \glsfirst{rsb} is to replace the uni-modal Gaussian with a learnable distribution that can approximate a complex distribution based on \gls{lars}~\cite{bauer2019resampled}. 
\gls{lars} iteratively re-weighs samples drawn a proposal distribution $\pi(\baseVar)$, e.g. a standard Gaussian, through a learned acceptance function $a_{\baseParam}: \mathcal{R}^{\featDim} \rightarrow [0,1]$.
To reduce the computation cost in practice, this process is truncated by accepting the $T$-th samples if the previous $T-1$ samples get rejected. 
% The resulting distribution is as follows:
% \begin{equation}
%     \label{rsb_base}
%     p_{\baseParam}(\baseVar) = (1 - \alpha_T)\frac{a_{\baseParam}(\baseVar)\pi(\baseVar)}{Z} + \alpha_T\pi(\baseVar)
% \end{equation}, 
To take into account conditional information, we need to conditionalize the learnable acceptance function $a_{\baseParam}(\baseVar)$ by modifying the output dimension of the acceptance function  $a_{\baseParam}(\baseVar)$ to predict the acceptance rate for each class. 
With this extension, we have the following conditional base distribution:
\begin{equation}
    \label{rsb_base}
    p_{\baseParam}(\baseVar|y=k) = (1 - \alpha_T)\frac{a_{\baseParam}(\baseVar)\pi(\baseVar|y_k)}{Z_k} + \alpha_T\pi(\baseVar),
\end{equation} 
where $a_{\baseParam}: \mathcal{R}^{\featDim} \rightarrow [0,1]^{C}$ and $\alpha_T = (1-Z)^{T-1}$, where Z is the normalization factor for $\pi(\baseVar)a_{\baseParam}(\baseVar)$, which can be estimated via Monte Carlo Sampling.
\paragraph{Discussion} There is another way to conditionalize the acceptance function by making the input $\baseVar$ conditioning on the class.  
However, this way requires higher computation overhead, i.e. multiple forward passes for each class when we need a marginalized base density for \gls{ood} detection (see sub-sec. \ref{inference}). 
Moreover, we did not observe much performance gain with this way in the preliminary experiments.
On the other hand, inspired by the \gls{gm}, we also tested class conditional Gaussians for the proposal distribution $\pi(\baseVar)$.
However, the hypothesized expressiveness did not covert to good performance in the preliminary experiments, we leave the investigation of this as future work.

% \subsubsection{\gls{ib} for conditional \gls{nf}}
% Class conditional information is valuable for accurate density estimation of data with semantic class labels e.g. $p(\featVar|\bb{y})$.
\subsubsection{Training with Information Bottleneck}
Directly training \gls{nf} with a conditional base distribution can lead to underperformance as observed in preliminary experiments and reported by~\citet{fetaya2019understanding}.
This attributes to the lack of explicit control for the balance between generative and discriminative modelling in the likelihood-based training objective of \gls{nf}.
To alleviate this, \gls{ib} provides a principle and explicit way to coordinate the influences from two different variables, e.g. $\featVarCap$ and $Y$ for learning the latent variable $\baseVarCap$.
\gls{ib}~\cite{tishby2000information} is an information theoretic approach for extracting relevant information measured by \gls{mi} about one variable $Y$ from another one $\featVarCap$.
This relevant information is squeezed through a 'bottleneck' of the information flow between $\featVarCap$ and $Y$ in form of another latent variable $\baseVarCap$.
Therefore, \gls{ib} strives to minimize the \gls{mi} $I(\featVarCap, \baseVarCap)$ between $\featVarCap$ and $\baseVarCap$ and simultaneously maximize the \gls{mi} $I(\baseVarCap, Y)$ between $\baseVarCap$ and $Y$ with a trade-off parameter to balance the two aspects.
% \begin{equation}
%     \label{ib}
%     \mathcal{L}_{IB} = I(\featVarCap, \baseVarCap) - \beta I(\baseVarCap, Y) 
% \end{equation}.

However, \gls{ib} is not directly ready for adoption as it is problematic to estimate the \gls{mi} between the input variable $\featVarCap$ and the latent $\baseVarCap$ of a flow due to the deterministic and bijective mapping $\flowFunc_\flowParam$, which raises the issue of invalidity of the definition of joint distribution between $\featVarCap$ and $\baseVarCap$.
 To this end, we adopt a technique proposed by~\citet{ardizzone2020training} which injects a small amount of noise $\epsilon$ into the input $\featVarCap$ for valid density definition and introduces an asymptotically exact version of \gls{ib} by defining another function $\hat{I}(\cdot, \cdot)$ to measure the relevant information between two random variables (more details in appendix):
\def\IBJdet{|\det(J_{T_{\flowParam}^{-1}}(\featVar+\epsilon))|}
\def\IBbaseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)))}
\def\condIBbaseL{(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)|y))}
\def\SumCondIBbaseL{\sum_{y\prime}(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)|y\prime))}
\begin{equation}
    \label{ib_nf}
    \mathcal{L}_{IBNF} =  \hat{I}(\featVarCap, \baseVarCap) - \beta \hat{I}(\baseVarCap, Y) 
\end{equation}
with 
\begin{equation}
    \label{ci_yz}
     \hat{I}(\baseVarCap, Y) = \mathbb{E}_{p(y)}\left[ \log \frac{p_{\baseParam}(\baseVar|y)p(y)}{\sum_{y\prime}(p_{\baseParam}(\baseVar|y\prime)p(y\prime))} \right] 
\end{equation}
and
\begin{equation}
    \label{ci_xz}
    \hat{I}(\featVarCap, \baseVarCap)=\mathbb{E}_{p(\featVar), p(\epsilon)}\left[ - \log {\sum_{y\prime}(p_{\baseParam}(\baseVar|y\prime))} - \log \IBJdet \right],
\end{equation}
where $\baseVar=\flowFunc_{\flowParam}^{-1}(\featVar+\epsilon)$ and $p(\epsilon) = \mathcal{N}(0, \sigma^2 \mathcal{I}_{\featDim})$ is a zero-meaned Gaussian with variance $\sigma^2$.
$\beta$ is a trade-off parameter to balance the two aspects.
With the flexible conditional base distributions defined in Eq. \ref{rsb_base}, we can train \textit{topologically matched} \gls{nf} with \gls{ib} by substituting \gls{crsb} into the conditional base probability $p_{\flowParam}(\baseVar|y)$ in Eq. \ref{ci_yz}.
More noteworthy, the \gls{ib} can better regularize the acceptance rate learning for \gls{crsb} to better assimilate the topological structure of the target distribution, leading to an overall improved performance on accurately approximating the complex target distribution ( see Fig. \ref{fig:rings_crsb_acceptance}). 

\subsection{Detecting OOD Objects}
\label{inference}
During test time, we detect the \gls{ood} objects based on the \glsfirst{ll} estimated from the topologically matched \gls{nf} trained with \gls{ib} as described in previous sub-sections.
As we model the complicated \gls{id} with \gls{nf}, the expected \gls{ll} for \gls{id} objects should be higher than \gls{ood} ones. 
A threshold to distinguish \gls{id} and \gls{ood} objects can be estimated from the training set. 
% For evaluation, to sidestep the influences of various selected thresholds, we measure the performance with \gls{auroc}. 
We marginalize over classes for the base distribution defined in Eq. \ref{rsb_base} and compute the final \gls{ll} based on the Change-of-Variables formula given the logits $\pb{\featVar}$ from the image and the object bounding box $\{ \pb{x}$, $\pb{b} \}$:
\begin{equation}
    \label{test_ll}
    LL_{test}(\pb{\featVar})=\log {\sum_{y\prime}(p_{\baseParam}(\flowFunc_{\flowParam}^{-1}(\pb{\featVar})|y\prime))} - \log |\det(J_{T_{\flowParam}^{-1}}(\pb{\featVar}))|.
\end{equation}
